End-to-End Visual Editing with a Generatively Pre-Trained Artist

We consider the targeted image editing problem: blending a region in a source image with a driver image that specifies the desired change. Differently from prior works, we solve this problem by learning a conditional probability distribution of the edits, end-to-end. Training such a model requires addressing a fundamental technical challenge: the lack of example edits for training. To this end, we propose a self-supervised approach that simulates edits by augmenting off-the-shelf images in a target domain. The benefits are remarkable: implemented as a state-of-the-art auto-regressive transformer, our approach is simple, sidesteps difficulties with previous methods based on GAN-like priors, obtains significantly better edits, and is efficient. Furthermore, we show that different blending effects can be learned by an intuitive control of the augmentation process, with no other changes required to the model architecture. We demonstrate the superiority of this approach across several datasets in extensive quantitative and qualitative experiments, including human studies, significantly outperforming prior work.

==> tables/LSUN_bedroom.tex <==
\begin{table}
\resizebox{\linewidth}{!}{
\begin{tabular}{m{3.5cm}lllllllllll}
\toprule
              & \multicolumn{2}{c}{FID \colorbox{lavenderblue}{($\downarrow$)}}                  & \multicolumn{2}{c}{Diversity (LPIPS) \colorbox{mistyrose}{($\uparrow$)}} & \multicolumn{3}{c}{Patch Retrieval \colorbox{mistyrose}{($\uparrow$)}}    & \multicolumn{2}{c}{Input Reconstruction \colorbox{lavenderblue}{($\downarrow$)}}    \\ \hline
                     & \multicolumn{2}{l}{Inception distribution} & \multicolumn{2}{l}{LPIPS distance}    & \multicolumn{3}{l}{Inception features} & \multicolumn{2}{l}{L1 Outside Edit-Region}    &                                          \\
                & Image             & Edit-Region            & Image          & Edit-Region          & R@1         & R@5        & R@20        & Real            & VQGAN              \\ \midrule

In-Domain (E)~\cite{zhu2020indomain}       &    44.027   &    43.544       & -          & -   & 0.171       &    0.363   & 0.608     &    0.208                                  &    -  \\
In-Domain (E+O) ~\cite{zhu2020indomain}      &    44.021   &    50.110       & -          & -   & 0.709       &    0.826   & 0.920     &    0.332                                  &    -  \\
EdiBERT~\cite{issenhuth2021edibert}        &   49.042    &   41.681        &    0.320       &   0.557     &  0.124      &  0.318     & 0.545     &  0.125                                    &  0.111    \\
Method 3        &       &           &           &        &       &       &      &                                      &      \\ \midrule 
Ours        &   44.021    &      22.749     &     0.304      &    0.471    &  0.531     & 0.757  &    0.905   & 0.121                                     &   0.104   \\\bottomrule
 
\end{tabular}
}
\caption{}
\end{table}

% 0.9228515625 0.9765625 0.984375 0.9931640625

==> tables/clothing_main.tex <==
\begin{table}
\resizebox{\linewidth}{!}{
\begin{tabular}{m{2.8cm}llllllllllllll}
\toprule
         &          & &            & \multicolumn{2}{c}{FID \colorbox{lavenderblue}{($\downarrow$)}}                    & \multicolumn{2}{c}{Diversity (LPIPS) \colorbox{mistyrose}{($\uparrow$)}} & \multicolumn{3}{c}{Patch Retrieval \colorbox{mistyrose}{($\uparrow$)}}    & \multicolumn{2}{c}{Input Reconstruction \colorbox{lavenderblue}{($\downarrow$)}}    & \multicolumn{1}{c}{NLL \colorbox{lavenderblue}{($\downarrow$)}}     & \\ \hline
            &   & &                & \multicolumn{2}{l}{Inception distribution} & \multicolumn{2}{l}{LPIPS distance}    & \multicolumn{3}{l}{Inception features} & \multicolumn{2}{l}{L1 Outside Edit-Region}    &                                          \\
         &      & &                & Image             & Edit-Region            & Image          & Edit-Region          & R@1         & R@5        & R@20        & Real            & VQGAN            & Paired Inputs                  & iters              \\ \midrule

\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Baselines and} \\ \colorbox{mistyrose}{\textbf{Upper}}/\colorbox{lavenderblue}{\textbf{Lower}}\\  \textbf{Bounds}\end{tabular}} & \multicolumn{3}{l}{ copy-paste}         &   30.131    &     59.048       &      0.093        &     0.348       &   0.978    &  0.997     &   1.000     &             0.000                                   &    0.049   & -   & -                     \\
& \multicolumn{3}{l}{copy-paste VQGAN }           &   31.569     &      58.589     &    0.091     &     0.343        &      \colorbox{mistyrose}{0.974}   &   \colorbox{mistyrose}{0.995}    & \colorbox{mistyrose}{1.000}     &          \colorbox{lavenderblue}{0.049}              &    \colorbox{lavenderblue}{0.000}   & -            & -                   \\

& \multicolumn{3}{l}{unconditional inpaint }  &    \colorbox{lavenderblue}{18.384}     &        \colorbox{lavenderblue}{22.956}       &      0.194          &        0.418              &    0.079        &  0.228         &     0.530       &     0.089 & 0.082 & 1.578 (?) & 2.6            \\ \midrule
\multirow{1}{*}{\textbf{Image Collaging}} & \multicolumn{3}{l}{EdiBERT~\cite{issenhuth2021edibert}}                  &    24.875     &        35.619       &      0.161          &    0.411                  &   0.104         &  0.267         &     0.554       &       0.057 & 0.047  & -                                          &    -                                        \\  \midrule
\multirow{9}{*}{\textbf{Ours}}& \multicolumn{3}{l}{EdiBERT ++ }            &    TODO     &        TODO       &  TODO              &         TODO             &     TODO       &       TODO    &    TODO        &         TODO                      &                              TODO  & TODO            \\ \cline{2-15}
&          Box-Ratio     & pos-aug  &  size-aug    & &           &         &                 &       &       &            &                                                 &       &         &                      \\\cline{2-4}
& 0.8 & \xmark &   \xmark            &    18.389     &             30.537  &      0.143          &    0.312                  &    0.636        &  0.855         &         0.961   &            0.058                                        &      0.049  &   2.169        &             25.3                \\
& 0.6 & \xmark &   \xmark           &  18.386       &     30.989          &        0.147        &      0.327                &     0.734       &    0.904       &       0.971     &     0.057                               &           0.049 & 1.700 & 2.6                                 \\
& 0.4 &\xmark &     \xmark     &   18.386      &        28.513       &          0.153      &        0.353              &    0.680        &  0.881         &     0.967       & 0.057                   & 0.048 &  1.594 &    -                                        \\
& 0.6 & \checkmark &   \xmark     &  18.386       &    28.301           &  0.154              &    0.355                  &        0.678    &  0.879         &     0.963       &       0.058              &      0.049 & 1.518 & 1.6                                      \\
& 0.5-0.6&\checkmark &     \checkmark           &    18.385     &    27.490           &      0.156          &        0.364           &    0.666        & 0.858          &     0.952       &  0.057                                    & 0.049 & 1.463              &  -                             \\  
& 0.4-0.7 & \checkmark &     \checkmark              &   18.387   & 25.551 & 0.156 & 0.365 & 0.595 & 0.802 & 0.925 & 0.057 & 0.048 & 1.449 &1.6        \\         
\bottomrule       
% & 0.8 & \xmark &   \xmark            &    18.387     &             31.695  &      0.154          &    0.341                  &    0.700        &  0.889         &         0.968   &            0.059                                        &      0.050  &   1.983        &             2.6                \\
% & 0.6 & \xmark &   \xmark           &  18.386       &     30.571          &        0.151        &      0.338                &     0.754       &    0.914       &       0.975     &     0.058                               &           0.049 & 1.700 & 2.6                                 \\
% & 0.4 &\xmark &     \xmark     &   18.386      &        28.891       &          0.156      &        0.356              &    0.603        &  0.827         &     0.949       & 0.058                   & 0.050 &  1.652 &    2.6                                        \\
% & 0.6 & \checkmark &   \xmark     &  18.386       &    27.000           &  0.161              &    0.369                  &        0.655    &  0.860         &     0.957       &       0.059              &      0.051 & 1.616 & 1.6                                      \\
% & 0.5-0.6&\checkmark &     \checkmark           &    18.387     &    26.048           &      0.160          &        0.372              &    0.641        & 0.840          &     0.941       &  0.058                                    & 0.049 & 1.535              &  1.6                             \\  
% & 0.4-0.7 & \checkmark &     \checkmark              &   18.385   & 24.515 & 0.164 & 0.380 & 0.523 & 0.753 & 0.904 & 0.058 & 0.050 & 1.590 &1.6        \\         
% \bottomrule    
\end{tabular}
}
\caption{these baselines are quite nuanced. So for FID, it is important that the same number of images are evaluated. For the generative models, it is 10240 images, but for the baselines, it was only 1024 because there was no variation. As you increase the number of images, FID decreases. So one option would be to use 10240 different images, but that would see far more variation than the generators who are only really seeing 1024 different ones. So scrap the copy-paste full, and instead use only the realistic one, and copy the patch at many different locations in the box. ALSO TO INCREASE THE RECALL - SIMPLY SAMPLE MANY AND PICK THE 10 MOST SIMILAR - JUST LIKE CLIP DOES. CHECK WHY UNCONDITIONAL DOES SO WELL ON PATCH RETRIEVAL (might be the sweep for most likley that I do). Additional analysis - view the attention maps to the conditional inputs (question to Andrea - is there a good way to do this? Perhaps aggregated attention softmax scores?  Need to change this because the patches in the val set are taken at a certain box ratio, which is unfair. Also check the box ratio on the saved image inputs (looks too small). For making BERT better, try completely dropping the black tokens (in the input), and varying how many iterations are done on the images, and check the collaging. Additionally try not blacking out the background at all and simply pasting the patch in at different sizes  \todo{have to re-evaluate these because the validation was not done properly - only paired NLL actually - also, implement improved sampling and the retrieval boosting}. \todo{When comparing to paint-by-word - explain how these feature-driven approaches cannot do fine-grained editing because the editing is being driven by a single aggregated feature that has become invariant to the fine-grained details for reconstruction.}}
\end{table}

% 0.9228515625 0.9765625 0.984375 0.9931640625



\begin{table}
\resizebox{\linewidth}{!}{
\begin{tabular}{m{2.8cm}llllllllllllll}
\toprule
         &          & &            & \multicolumn{2}{c}{FID \colorbox{lavenderblue}{($\downarrow$)}}                    & \multicolumn{2}{c}{Diversity (LPIPS) \colorbox{mistyrose}{($\uparrow$)}} & \multicolumn{3}{c}{Patch Retrieval \colorbox{mistyrose}{($\uparrow$)}}    & \multicolumn{2}{c}{Input Reconstruction \colorbox{lavenderblue}{($\downarrow$)}}    & \multicolumn{1}{c}{NLL \colorbox{lavenderblue}{($\downarrow$)}}     & \\ \hline
            &   & &                & \multicolumn{2}{l}{Inception distribution} & \multicolumn{2}{l}{LPIPS distance}    & \multicolumn{3}{l}{Inception features} & \multicolumn{2}{l}{L1 Outside Edit-Region}    &                                          \\
         &      & &                & Image             & Edit-Region            & Image          & Edit-Region          & R@1         & R@5        & R@20        & Real            & VQGAN            & Paired Inputs                  & iters              \\ \midrule

\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Baselines and} \\ \colorbox{mistyrose}{\textbf{Upper}}/\colorbox{lavenderblue}{\textbf{Lower}}\\  \textbf{Bounds}\end{tabular}} & \multicolumn{3}{l}{ copy-paste}         &   30.131    &     59.048       &      0.093        &     0.348       &   0.978    &  0.997     &   1.000     &             0.000                                   &    0.049   & -   & -                     \\
& \multicolumn{3}{l}{copy-paste VQGAN }           &   31.569     &      58.589     &    0.091     &     0.343        &      \colorbox{mistyrose}{0.974}   &   \colorbox{mistyrose}{0.995}    & \colorbox{mistyrose}{1.000}     &          \colorbox{lavenderblue}{0.049}              &    \colorbox{lavenderblue}{0.000}   & -            & -                   \\

& \multicolumn{3}{l}{unconditional inpaint }  &    \colorbox{lavenderblue}{18.384}     &        \colorbox{lavenderblue}{22.956}       &      0.194          &        0.418              &    0.079        &  0.228         &     0.530       &     0.089 & 0.082 & 1.578 (?) & 2.6            \\ \midrule
\multirow{1}{*}{\textbf{Image Collaging}} & \multicolumn{3}{l}{EdiBERT~\cite{issenhuth2021edibert}}                  &    24.875     &        35.619       &      0.161          &    0.411                  &   0.104         &  0.267         &     0.554       &       0.057 & 0.047  & -                                          &    -                                        \\  \midrule
\multirow{2}{*}{\textbf{Ours}}& \multicolumn{3}{l}{EdiBERT ++ }            &    TODO     &        TODO       &  TODO              &         TODO             &     TODO       &       TODO    &    TODO        &         TODO                      &                              TODO  & TODO            \\ 
&  & \multicolumn{2}{l}{(Ours) \method} &     18.387   & 25.551 & 0.156 & 0.365 & 0.595 & 0.802 & 0.925 & 0.057 & 0.048 & 1.449 &1.6        \\         
\bottomrule       
% & 0.8 & \xmark &   \xmark            &    18.387     &             31.695  &      0.154          &    0.341                  &    0.700        &  0.889         &         0.968   &            0.059                                        &      0.050  &   1.983        &             2.6                \\
% & 0.6 & \xmark &   \xmark           &  18.386       &     30.571          &        0.151        &      0.338                &     0.754       &    0.914       &       0.975     &     0.058                               &           0.049 & 1.700 & 2.6                                 \\
% & 0.4 &\xmark &     \xmark     &   18.386      &        28.891       &          0.156      &        0.356              &    0.603        &  0.827         &     0.949       & 0.058                   & 0.050 &  1.652 &    2.6                                        \\
% & 0.6 & \checkmark &   \xmark     &  18.386       &    27.000           &  0.161              &    0.369                  &        0.655    &  0.860         &     0.957       &       0.059              &      0.051 & 1.616 & 1.6                                      \\
% & 0.5-0.6&\checkmark &     \checkmark           &    18.387     &    26.048           &      0.160          &        0.372              &    0.641        & 0.840          &     0.941       &  0.058                                    & 0.049 & 1.535              &  1.6                             \\  
% & 0.4-0.7 & \checkmark &     \checkmark              &   18.385   & 24.515 & 0.164 & 0.380 & 0.523 & 0.753 & 0.904 & 0.058 & 0.050 & 1.590 &1.6        \\         
% \bottomrule    
\end{tabular}
}

\end{table}

\begin{table}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllllllllllllll}
\toprule
           &      & &            & \multicolumn{2}{c}{FID \colorbox{lavenderblue}{($\downarrow$)}}                    & \multicolumn{2}{c}{Diversity (LPIPS) \colorbox{mistyrose}{($\uparrow$)}} & \multicolumn{3}{c}{Patch Retrieval \colorbox{mistyrose}{($\uparrow$)}}    & \multicolumn{2}{c}{Input Reconstruction \colorbox{lavenderblue}{($\downarrow$)}}    & \multicolumn{1}{c}{NLL \colorbox{lavenderblue}{($\downarrow$)}}     & \\ \hline
         & & &                & \multicolumn{2}{l}{Inception distribution} & \multicolumn{2}{l}{LPIPS distance}    & \multicolumn{3}{l}{Inception features} & \multicolumn{2}{l}{L1 Outside Edit-Region}    &                                          \\
          &    & &                & Image             & Edit-Region            & Image          & Edit-Region          & R@1         & R@5        & R@20        & Real            & VQGAN            & Paired Inputs                  & iters              \\ \midrule
      model     & top-k  &  top-p & filter   & &           &         &                 &       &       &            &                                                 &       &         &                      \\\cline{2-4}
   ver-6 &  50 &     -    & -    &    18.386     &             24.913  &      0.152          &    0.356                  &    0.616        &  0.825         &         0.930   &            0.057                                        &      0.048  &   1.444       &             25.3                \\
 ver-6 &  100 &     - & -       &    18.389     &             25.654  &      0.156          &    0.366                  &    0.596        &  0.809         &         0.927   &            0.057                                        &      0.048  &   1.444       &             25.3                \\
  ver-6 &  200 &        - & -     &    18.386     &             26.228  &      0.159          &    0.373                  &    0.583        &  0.791         &         0.915   &            0.057                                        &      0.049  &   1.444       &             25.3                \\
    
    ver-6 &  400 &          - & -      &    18.386     &             26.576  &      0.160          &    0.377                  &    0.572        &  0.781         &         0.912   &            0.057                                        &      0.049  &   1.444       &             25.3                \\
    ver-6 &  - &     0.95      & -      &    18.386     &             25.083  &      0.151          &    0.359                  &    0.599        &  0.804         &         0.923   &            0.057                                        &      0.047  &   1.444       &             25.3                \\
    
    ver-6 &  - &     0.90       & -     &    18.386     &             24.420  &      0.144          &    0.348                  &    0.615        &  0.817         &         0.927   &            0.056                                        &      0.046  &   1.444       &             25.3                \\
    ver-6 &  - &     0.85      & -      &    18.386     &             23.964  &      0.139          &    0.340                  &    0.623        &  0.826         &         0.930   &            0.056                                        &      0.046  &   1.444       &             25.3                \\
    ver-6 &  - &     0.825       & -     &    18.386     &             23.931  &      0.137          &    0.336                  &    0.628        &  0.827         &         0.931   &            0.055                                        &      0.045  &   1.444       &             25.3                \\
    ver-6 &  - &     0.80       & -     &    18.386     &             23.811  &      0.134          &    0.332                  &    0.627        &  0.830         &         0.933   &            0.055                                        &      0.045  &   1.444       &             25.3                \\
    ver-6 &  - &     0.75       &      &    18.386     &             23.714  &      0.129          &    0.325                  &    0.646        &  0.833         &         0.938   &            0.055                                        &      0.045  &   1.444       &             25.3                \\
    ver-6 &  - &     0.65       &      &    18.386     &             23.834  &      0.121          &    0.312                  &    0.650        &  0.837         &         0.939   &            0.055                                        &      0.044  &   1.444       &             25.3                \\
     ver-6 &  - &     0.60       &      &    18.386     &             23.677  &      0.117          &    0.306                  &    0.647        &  0.837         &         0.935   &            0.055                                        &      0.044  &   1.444       &             25.3                \\
     ver-6 &  - &     0.50       &      &    18.386     &             23.836  &      0.109          &    0.293                  &    0.658        &  0.842         &         0.940   &            0.055                                        &      0.044  &   1.444       &             25.3                \\
     ver-6 &  - &     0.40       &      &    18.386     &             23.966  &      0.101          &    0.281                  &    0.664        &  0.839         &         0.939   &            0.055                                        &      0.044  &   1.444       &             25.3                \\
    ver-6 &  - &     0.80       & 20-10     &    18.386     &             24.351  &      0.132          &    0.326                  &    0.799        &  0.932         &         0.979   &            0.055                                        &      0.045  &   1.444       &             25.3                \\
ver-6 &  - &     0.80       & 40-10     &    18.386     &             24.489  &      0.132          &    0.324                  &    0.876        &  0.965         &         0.991   &            0.055                                        &      0.045  &   1.444       &             25.3                \\
ver-6 &  - &     0.80       & 100-10     &    18.386     &             24.794  &      0.131          &    0.322                  &    0.934        &  0.985         &         0.996   &            0.055                                        &      0.045  &   1.444       &             25.3                \\

    

\bottomrule       

\end{tabular}
}
\caption{sweeping over sampling methods. top - k : top-k sampling from the model (at each step, the model samples from the k tokens with highest probability). top-p : top-p sampling where at each step the model sampels from the tokens whose cumulative probability sums to p. filter: This is where you make more samples, but only consider those that were most similar to the visual cue. These sampling methods give very big boosts to quality and retrieval metrics over the naive sampling used previously}
\end{table}
